Listwise Preference Diffusion Optimization for User Behavior Trajectories Prediction

Forecasting multi-step user behavior trajectories requires reasoning over structured preferences across future actions, a challenge overlooked by traditional sequential recommendation. This problem is critical for applications such as personalized commerce and adaptive content delivery, where anticipating a user's complete action sequence enhances both satisfaction and business outcomes. We identify an essential limitation of existing paradigms: their inability to capture global, listwise dependencies among sequence items. To address this, we formulate User Behavior Trajectory Prediction (UBTP) as a new task setting that explicitly models long-term user preferences. We introduce Listwise Preference Diffusion Optimization (LPDO), a diffusion-based training framework that directly optimizes structured preferences over entire item sequences. LPDO incorporates a Plackett-Luce supervision signal and derives a tight variational lower bound aligned with listwise ranking likelihoods, enabling coherent preference generation across denoising steps and overcoming the independent-token assumption of prior diffusion methods. To rigorously evaluate multi-step prediction quality, we propose the task-specific metric Sequential Match (SeqMatch), which measures exact trajectory agreement, and adopt Perplexity (PPL), which assesses probabilistic fidelity. Extensive experiments on real-world user behavior benchmarks demonstrate that LPDO consistently outperforms state-of-the-art baselines, establishing a new benchmark for structured preference learning with diffusion models.

==> main_table.tex <==
\begin{table*}[ht]
    \small
 \caption{Overall performance. Bold scores represent the highest results of all methods. Underlined scores stand for the second-highest results. Our model achieves the state-of-the-art result among all baseline models. $^*$ means the improvement is significant at $p < 0.05$, with the relative improvements denoted as Improv.}
 \vspace{-1em}
    \centering
    \resizebox{\textwidth}{!}{
     \begin{tabular}{c|l|cccc|ccc|ccc|c|c}
     \toprule
          Dataset& Metric                &GRU4Rec  &Caser &SARSRec &BERT4Rec & S$^3$Rec &CL4SRec & ICLRec & DreamRec & DiffuRec &SdifRec & \textbf{\Model} & Improv.\\
          \midrule                       
          \multirow{4}*{Beauty} &HR@5    &0.0363 &0.0374 &0.0337 &0.0209 &0.0189 &0.0423 &0.0493 &0.0498 &0.0559 &\underline{0.0609} &$\textbf{0.0630}^*$&3.45\%\\
                                &HR@10   &0.0571 &0.0601 &0.0635 &0.0393 &0.0307 &0.0694 &0.0737 &0.0698  &0.0783& \underline{0.0819} &$\textbf{0.0859}^*$&4.88\%\\
                                &NDCG@5  &0.0243 &0.0241 &0.0237 &0.0110 &0.0115 &0.0281 &0.0324 &0.0325 &0.0406 &\underline{0.0437}  &$\textbf{0.0449}^*$&2.74\%\\
                                &NDCG@10 &0.0310 &0.0332 &0.0322 &0.0169 &0.0153 &0.0373 &0.0393 &0.0397 &0.0478 &\underline{0.0507} &$\textbf{0.0523}^*$&3.16\%\\
         \midrule                       
         \multirow{4}*{Toys}    &HR@5   &0.0286 &0.0208 &0.0432 &0.0274 &0.0143 &0.0526 &0.0590  &0.0510 &0.0550& \underline{0.0588} &$\textbf{0.0690}^*$&17.35\%\\
                                &HR@10  &0.0440 &0.0322 &0.0660 &0.0450 &0.0094 &0.0776 &0.0830  &0.0635 &0.0739& \underline{0.0758} &$\textbf{0.0903}^*$&19.13\%\\
                                &NDCG@5 &0.0179 &0.0135 &0.0293 &0.0174 &0.0123 &0.0362 &0.0403  &0.0316 &0.0411& \underline{0.0447} &$\textbf{0.0518}^*$&15.88\%\\
                                &NDCG@10&0.0228 &0.0172 &0.0347 &0.0231 &0.0391 &0.0428 &0.0479  &0.0391  &0.0471& \underline{0.0498} &$\textbf{0.0587}^*$&17.87\%\\
        \midrule                     
        \multirow{4}*{Yelp}     &HR@5   &0.0142 &0.0160 &0.0162 &0.0196 &0.0101 &0.0229 &0.0257   &0.0174 &\underline{0.0364}& 0.0233 &$\textbf{0.0405}^*$&11.26\%\\
                                &HR@10  &0.0248 &0.0254 &0.0311 &0.0339 &0.0176 &0.0392&0.0426    &0.0193 &\underline{0.0551}& 0.0375&$\textbf{0.0611}^*$&10.89\%\\
                                &NDCG@5 &0.0080 &0.0101 &0.0096 &0.0121 &0.0068 &0.0144 &0.0162   &0.0117 &\underline{0.0253}& 0.0157&$\textbf{0.0272}^*$&7.51\%\\
                                &NDCG@10&0.0124 &0.0113 &0.0136 &0.0167 &0.0092 &0.0197 &0.0217   &0.0152 &\underline{0.0313}& 0.0201&$\textbf{0.0338}^*$&7.99\%\\
        \bottomrule                  
     \end{tabular}
    }
     \label{tab:overall}
\end{table*}


